On Bounded Advice Classes

Advice classes in computational complexity have frequently been used to model real-world scenarios encountered in cryptography, quantum computing and machine learning, where some computational task may be broken down into a preprocessing and deployment phase, each associated with a different complexity. However, in these scenarios, the advice given by the preprocessing phase must still be generated by some (albeit more powerful) bounded machine, which is not the case in conventional advice classes. To better model these cases we develop `bounded advice classes', where a more powerful Turing machine generates advice for another, less powerful, Turing machine. We then focus on the question of when various classes generate useful advice, to answer this we connect bounded advice to unary languages. This connection allows us to state various conditional and unconditional results on the utility of advice generated by $\mathsf{EXP}$, $\mathsf{NP}$, $\mathsf{BQP}$, $\mathsf{PSPACE}$, and more. We study the relations between bounded advice classes, quantum bounded advice classes, and randomised bounded advice. We also examine how each of these concepts interact with recently introduced classes, like $\mathsf{BPP/samp}$. Our results also improve the state of the art in existing research on the complexity of advice functions.

==> sections/ConnectionToSparsity.tex <==
At the core of many of our results is a connection between bounded advice and sparsity, which the following theorem highlights. This section will focus on the proof of the following three main theorems without much narrative importance of them.

\begin{theorem}\label{thm: advice to sparsity}
    For any complexity class $\mathsf{B}$:
    $$
    \mathsf{P/poly^B \subseteq P^{SP(P^B)}}
    \text{ and }
    \mathsf{P^{SP(P^B)}} \subseteq \mathsf{P/poly^{NP^B}}
    $$
\end{theorem}

This theorem is central, but for two special cases ($\mathsf{PSPACE}$ and $\mathsf{NP}$) there exist tighter versions:

\begin{theorem}\label{thm: advice to sparsity, PSPACE-case}
    $$
    \mathsf{ P/poly^{PSPACE} = P^{SP(PSPACE)}}.
    $$
\end{theorem}

\begin{theorem} \label{thm: advice to sparsity, NP-case}
    $$
    \mathsf{P^{SP(NP)} = P/poly^{SP(NP)}}.
    $$
\end{theorem}

In the third subsection, we will discuss how this result might be improved to $\mathsf{P^{SP(P^{NP})} = P/poly^{NP}}$. The core problem is that we are able to show $\mathsf{NP^{SP(NP)}= P^{NP}}$ but unable to show a similar result for $\mathsf{NP^{SP(P^{NP})}}$.
\color{red}
However, this is closely related to NEXP not in P/poly. So must run into the same algebrization barriers that are known for this problem. Our result is closely related to Malaneys thm...

Could replace these with tally... 
\color{black}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Sparcity proof 1 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem \ref{thm: advice to sparsity}}

We break proving Theorem \ref{thm: advice to sparsity} into two lemmas, \ref{lma: Simple Poly oracle} \& \ref{cor: sparse in advice}.

\begin{lemma}\label{lma: Simple Poly oracle}
For all complexity classes $\mathsf{B}$ and $\mathsf{C}$:
    $$\mathsf{B/poly^C\subseteq P^{B, SP(P^C)}}.$$
\end{lemma}

The 


The first inclusion of Theorem \ref{thm: advice to sparsity}, $\mathsf{P/poly^B \subseteq P^{SP(P^B)}}$, is a special case of Lemma \ref{lma: Simple Poly oracle}, with $\mathsf{B=P}$ and $\mathsf{C=B}$. We state this in the following corollary.

\begin{corollary}
    For any complexity class $\mathsf{B}$:
    $$
    \mathsf{P/poly^B \subseteq P^{SP(P^B)}}
    $$
\end{corollary}

To finish the proof of Theorem \ref{thm: advice to sparsity} we must show $\mathsf{P^{SP(B)}} \subseteq \mathsf{P/poly^{NP^B}}$. We prove a stronger result in the following lemma and then provide the exact result in a corollary immediately after.

\begin{lemma} \label{lma: NP sparse containment}
    For complexity class $\mathsf{B}$:
    $$
    \mathsf{P^{SP(B) \hspace{0.1cm}}  \subseteq P/poly^{SP(NP^{SP(B)})}} 
    $$
\end{lemma}

\begin{proof}
    Let $K$ be a language in $\mathsf{P^{SP(B)}}$, there exists a sparse language, ${L}$ in $\mathsf{B}$ such that $K\in P^L$. For any $n$, as $L$ is sparse there are at most polynomially many strings $x\in L$ of length $n$. Our strategy will be to find all of these strings with the advice generating TM, to create a list, $A_n=\{x: x\in L, |x|\leq n\}$, and pass $A_n$ as advice. The advice using TM can then simulate an oracle call to $L$ by simply checking if $x$ is on the list.

    It is possible to generate $A_n$ in polynomial time with access to an $\mathsf{NP^B}$ oracle, with access to the language: 
    
    $$
    L'_{sparse} = \{
    1^n\#p: \exists x \text{ with } x\in L, \text{ and $p$ is a prefix of }x
    \}.
    $$

    We can use $L'_{sparse}$ to find a complete list of strings by beginning with an empty list, $A=\{\}$. Begin by using algorithm \ref{Alg:binary search variant} to find an initial element, $x\in L$, and put this element in $A$. If we try to nïavely reuse algorithm \ref{Alg:binary search variant} to find more elements it may not return a new value of $x\in L$. We must force the algorithm to return a new value of $x$. We can solve this problem to begin searching from some particular prefix, instead of from the empty string.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{trie_search.png}
    \caption{\textbf{Procedure for finding all the elements of a sparse language using $L'_{sparse}$.} We begin with a possibly incomplete list of $x\in L$, the list is called $A$. In step \textbf{a} we represent $A$ with a prefix tree, each layer representing a possible prefix of the string, if a string is a prefix for an element in $\mathsf{A}$ its branch continues to a green node. \textbf{b.} We add the possible unexplored children to the tree. We then use algorithm \ref{Alg:binary search variant} starting from each unexplored child prefixes to find possible new elements of $A$. Either one is found and added to $A$ (\textbf{d.}) or none are found, implying there are none left to find and $A$ is complete (\textbf{c.}).}
    \label{fig:trie search}
\end{figure}

    Suppose our list, $A$, has $m$ elements in it. This defines a partially explored trie, as shown in figure \ref{fig:trie search}. At each node there are two children, one child must be an explored path that leads to at least one previously found element of $x\in A$, the other child may be unexplored. By beginning the search with a prefix from the unexplored children (highlighted in step b of figure \ref{fig:trie search}) we will either find a previously unfound $x\in L$, which we can add to $A$, or we will find no new $x \in L$, and can assume that the list is complete $A=A_n$. As $A_n$ has at most polynomial elements and the tree is polynomially deep, finding each element takes at most polynomial time.

    Starting from the first element of $A$ we can repeat this process until $A$ is full. We then convert this list to a string and pass it as advice. Importantly, the language $L'_{sparse}$ is sparse, and the language $L \in B$ that is used to define $L'_{sparse}$ is also sparse. Giving us the sparsity requirements
\end{proof}

A special case of this lemma is the required result ($\mathsf{P/poly^B \subseteq P^{SP(P^B)}}$).

\begin{corollary} \label{cor: sparse in advice}
 For any complexity class, $\mathsf{B}$:
    $$ \mathsf{P^{SP(B)} \hspace{0.1cm}  \subseteq P/poly^{NP^B}}$$
\end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Sparcity PSPACE %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm: advice to sparsity, PSPACE-case}}
This subsection focuses on proving Theorem \ref{thm: advice to sparsity, PSPACE-case}, which we restate here

\addtocounter{theorem}{-6}
\begin{theorem}
    $$
    \mathsf{ P/poly^{PSPACE} = P^{SP(PSPACE)}}.
    $$
\end{theorem}
\addtocounter{theorem}{+5}

To prove this result we need the following lemma:
\begin{lemma}\label{lma: NP PSPACE in PSPACE}
    $\mathsf{NP^{PSPACE}=PSPACE}$
\end{lemma}
\begin{proof}
    $$
    \mathsf{PSPACE\subseteq NP^{PSPACE}\subseteq PSPACE^{PSPACE}}
    $$
    But as $\mathsf{PSPACE}$ is self-low
    $$\mathsf{PSPACE^{PSPACE} \subseteq PSPACE}$$
\end{proof}

We now proceed with the proof of Theorem \ref{thm: advice to sparsity, PSPACE-case}

\begin{proof}[Proof of Theorem \ref{thm: advice to sparsity, PSPACE-case}]
By Corollary \ref{cor: sparse in advice} 
$$
\mathsf{P^{SP(PSPACE)}}\subseteq \mathsf{P/poly^{NP^{PSPACE}}}.
$$
But as we have shown in lemma \ref{lma: NP PSPACE in PSPACE} $\mathsf{NP^{PSPACE}=PSPACE}$. Therefore,
    $$
    \mathsf{P^{SP(PSPACE)}\subseteq P/poly^{PSPACE}}.
    $$

    By Theorem \ref{thm: advice to sparsity} this inclusion also holds in the other direction.
    $$
    \mathsf{P/poly^{PSPACE} \subseteq P^{SP(PSPACE)}}
    $$
    Therefore $\mathsf{P/poly^{PSPACE}=P^{SP(PSPACE)}}$.
    
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Sparcity proof 3 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem \ref{thm: advice to sparsity, NP-case}}

This subsection adds proofs to an interesting special case of Theorem \ref{thm: advice to sparsity}, when $\mathsf{B=NP}$ ($\mathsf{NP}$ oracle advice generation) mentioned in the opening of this section. We restate this theorem:

\addtocounter{theorem}{-6}
\begin{theorem}
    $$
    \mathsf{P^{SP(NP)} = P/poly^{SP(NP)}}.
    $$
\end{theorem}
\addtocounter{theorem}{+5}

At the end of the subsection, we discuss how this case might be improved by future work.

The key piece to realising Theorem \ref{thm: advice to sparsity, NP-case} is the following lemma, which is (as far as the authors can tell) a novel result for sparse $\mathsf{NP}$ languages. The proof is a relatively simple census-based proof.

\begin{lemma}\label{lma:np sp np}
    For any complexity class $\mathsf{B}$
    $$
    \mathsf{NP^{SP(NP^B)}}\subseteq \mathsf{P^{NP^B}}
    $$
    Furthermore,
    $$
    \mathsf{SP(NP^{SP(NP^B)})}=
    \mathsf{SP(P^{SP(NP^B)})}
    $$
\end{lemma}
To prove this lemma we begin by showing the $\mathsf{SP(NP^{SP(NP^B)})}=\mathsf{SP( P^{SP(NP^B)})}$ equality. One direction of this equality is trivial: As $\mathsf{P\subseteq NP}$ relative to all oracles, $
\mathsf{SP(NP^{SP(NP^B)})} \supseteq
\mathsf{SP(P^{SP(NP^B)})}
$. The other direction of the inclusion is less obvious, to prove it we will use a similar proof to lemma \ref{lma: NP sparse containment}, describing a polynomial time procedure to find a list of all the elements of the $\mathsf{SP(NP^B)}$ oracle with access to a different $\mathsf{SP(NP^B)}$ oracle. 
Once this list is found we can provide it alongside $x$ as a call to an $\mathsf{NP}$ oracle to simulate the entire algorithm. We then prove $\mathsf{NP^{SP(NP^B)}}\subseteq \mathsf{P^{NP^B}}$ as a small modification.
\begin{proof}
    Let $K$ be a language in $\mathsf{SP(NP^{SP(NP^B)})}$, let $L\in \mathsf{SP(NP^B)}$ be a language such that $K\in \mathsf{SP(NP)}^L$ ($L$ is the oracle). As $L\in \mathsf{NP^B}$, we can write it as a quantified formula with reference to a new language $L_{P^B} \in \mathsf{P^B}$:

    $$
    L = \{ x:
    \exists c \hspace{0.1cm} x\#c \in L_{P^B}
    \}
    $$

    We would like to find all the elements of size $n$ of this language and add them to a list, $A_n$. Writing $L$ in the quantified boolean form allows us to do this with another $\mathsf{NP^B}$ language:

    $$
    L' = \{1^n\# p: \exists y \exists x \hspace{0.1cm} p \text{ is a prefix of }x, x\#y \in L_{P^B}
    \}
    $$

    As the two existence quantifiers are next to each other we can combine them into a single quantifier, placing the language in $\mathsf{NP^B}$. Furthermore, as there are only polynomially many prefixes of possible elements of $L$, this language is sparse. 

    We can search over the prefixes of $L'$ to find all $x\in L$ up to a certain size in polynomial time, exactly as described in Lemma \ref{lma: NP sparse containment}(/figure \ref{fig:trie search}). 
    Assuming we now have a list of all the elements of $L$ up to a certain size it is relatively simple to compute $K(x)$. As $K \in \mathsf{SP(NP)}^L$ once the list is provided, we can decide if any $x$ is in $K$ with another oracle call to an $\mathsf{SP(NP)}$ language, placing $K\in \mathsf{P^{SP(NP^B)}}$
    %footnote
    \footnote{Technically we have shown $K\in \mathsf{P^{SP(NP^B), SP(NP^B)}}$ as the final oracle call will likely not call the same language as we use to find the elements of $L$. However, for any two sparse languages, $L_1, L_2\in \mathsf{NP^B}$ there exists a third, sparse language in $\mathsf{NP^B}$, 
    which can decide either language by using one extra bit to mark which language it is to decide.}.
    %end footnote
    This completes the proof of the equality $\mathsf{SP(NP^{SP(NP^B)})}=
    \mathsf{SP(P^{SP(NP^B)})}$.

    To show $\mathsf{NP^{SP(NP^B)}}\subseteq \mathsf{P^{SP(NP^B)}}$, we can repeat the procedure to find all elements of the oracle $L$ using the language $L'$, however now we must use a non-sparse call to a $\mathsf{NP}$ language as the final call to decide $K$.
\end{proof} 

While the previous lemma is not a result in bounded advice classes, it makes the proof of Theorem \ref{thm: advice to sparsity, NP-case} quite simple. In fact, the strength of Lemma \ref{lma:np sp np} allows us to prove a stronger result than Theorem \ref{thm: advice to sparsity, NP-case}, one which characterises sparse advice from the whole polynomial hierarchy, instead of just from the $\mathsf{NP}$ layer. 

\begin{theorem}\label{thm: sparcity in advice, poly hierarchy}
    For all $i>0$:
    $$
    \mathsf{P^{SP(\Sigma_i^P)}  \subseteq P/poly^{SP(\Sigma_i^P)}} 
    $$
\end{theorem}
\begin{proof}
    Using Lemma \ref{lma: NP sparse containment} with $\mathsf{B=\Sigma_i^P}$, we get the inequality:
    $$
    \mathsf{P^{SP(\Sigma_i^P)}} \subseteq \mathsf{P/poly^{SP(NP^{SP(\Sigma_i^P)})}}.
    $$
    We can transform this expression by writing $\mathsf{\Sigma_{i}^P = NP^{\Sigma_{i-1}^P}}$,
    $$
    \mathsf{P^{SP(\Sigma_i^P)}} \subseteq \mathsf{P/poly^{SP(NP^{SP(NP^{\Sigma_{i-1}^P})})}}.
    $$
    By Lemma \ref{lma:np sp np}, $\mathsf{SP(NP^{SP(NP^{\Sigma_{i-1}^P})})\subseteq P^{SP(NP^{\Sigma_{i-1}^P})}}$, therefore:
    $$
    \mathsf{P^{SP(\Sigma_i^P)}} \subseteq \mathsf{P/poly^{ P^{SP(NP^{\Sigma_{i-1}^P})}}}
    $$
    Rewriting $\mathsf{NP^{\Sigma_{i-1}^P}=\Sigma_{i}^P}$ we get 
    $$
    \mathsf{P^{SP(\Sigma_i^P)}}
    \subseteq
    \mathsf{P/poly^{P^{SP(\Sigma_i^P)}}}.
    $$
    Finally, we absorb this $\mathsf{P}$ into the polynomial advice generator to arrive at the final result.      
\end{proof}

This direction of the proof is only a relatively small improvement on lemma 6 of \cite{Ko85Circuit-Size}, stating this lemma in the notation developed here: $\mathsf{\Sigma_i^P\subseteq P/poly^{\Sigma_i^P}}$. The addition of the sparsity on the right-hand side is a key insight necessary for the final result (of which Theorem \ref{thm: advice to sparsity, NP-case} is the $i=1$ case).

\begin{corollary}\label{cor: sparcity to advice, poly hierarchy}
    For all $i\geq 0$
    $$
     \mathsf{P^{SP(\Sigma_i^P) \hspace{0.1cm}}  = P/poly^{SP(\Sigma_i^P)}} 
    $$
\end{corollary}
\begin{proof}
By theorem \ref{thm: sparcity in advice, poly hierarchy}
    $$
     \mathsf{P^{SP(\Sigma_i^P) \hspace{0.1cm}}  \subseteq P/poly^{SP(\Sigma_i^P)}}.
    $$
By theorem \ref{thm: advice to sparsity}
    $$
     \mathsf{ P/poly^{SP(\Sigma_i^P)}  \subseteq
     P^{SP(\Sigma_i^P) \hspace{0.1cm}}}.
    $$
\end{proof}

As $\mathsf{P/poly^{NP}}=\mathsf{P/poly^{SP( P^{NP})}}$, if this result could be modified to hold for $\mathsf{P^{NP}}$ instead of $\mathsf{NP}$ then we would have the meaningful connection: $\mathsf{P/poly^{NP}= P^{SP(P^{NP})}}$. 
However, proving this may be immensely difficult as it would likely also imply that under the assumption $\mathsf{NEXP\subseteq P/poly}$ that $\mathsf{\mathsf{EXP^{NP}=NEXP}}$, the key step in showing the contradiction and thus that $\mathsf{NEXP \not \subseteq P/poly}$. A result which is known to have some of the hardest barriers in complexity theory \cite{aaronson2009algebrization}.

==> sections/trashcan.tex <==
---
Another important use of quantum complexity classes is in the class $\mathsf{BPP/SAMP(BQP)}$ \cite{cite}, where samples from a quantum computer are used to aid a classical probabilistic time algorithm. As the computation that is being sampled from can be chosen at will this class is equal to $\mathsf{BPP/poly^{BQP}}$.

\begin{lemma}
    $$
    \mathsf{BPP/samp(BQP)=BPP/poly^{BQP}}
    $$
\end{lemma}

Using the $\mathsf{BPP}$ variant of Theorem \ref{thm: advice is unary}:

\begin{theorem}
    $$
    \mathsf{BPP/samp(BQP)=BPP^{Un(BQP)}}
    $$
\end{theorem}
\begin{proof}
    \textbf{Claim 1: $\mathsf{BPP/poly^{BQP}\subseteq BPP^{Un(BQP)}}$}
    
    By Lemma \ref{lma: advice in unary},
    $$
    \mathsf{ BPP/poly^{BQP}\subseteq P^{BPP, Un(P^{BQP})}}
    $$
    We can simplify this, note $\mathsf{P^{BQP}=BQP}$ and $\mathsf{P^{BPP}=BPP}$.
    $$
    \mathsf{BPP/poly^{BQP}\subseteq BPP^{Un(BQP)}}
    $$

    \textbf{Claim 2: $\mathsf{BPP^{Un(BQP)} \subseteq BPP/poly^{BQP}}$}
    A proof of this claim is almost a direct repeat of Lemma \ref{lma: unary in advice}. We use the $\mathsf{BQP}$ advice generator to resolve each $1^n$ for all $n$ up to the input size. Passing this as advice allows the $\mathsf{BPP}$ advice receiver to simulate oracle calls to the unary $\mathsf{BQP}$ language.

    Together Claims 1 and 2 prove $\mathsf{BPP^{Un(BQP)} = BPP/poly^{BQP}}$, as $\mathsf{BPP/samp(BQP)=BPP^{Un(BQP)}}$ the result is proved.
\end{proof}

This is interesting as it shows that the unary languages used by \cite{cite} to show $\mathsf{BPP/samp}$ is not just $\mathsf{BPP}$ are in fact all the languages reachable by $\mathsf{BPP/samp}$.
